Adaptive Decontamination of the Training Set: A Unified Formulation for Discriminative Visual Tracking

Tracking-by-detection methods have demonstrated competitive performance in recent years. In these approaches, the tracking model heavily relies on the quality of the training set. Due to the limited amount of labeled training data, additional samples need to be extracted and labeled by the tracker itself. This often leads to the inclusion of corrupted training samples, due to occlusions, misalignments and other perturbations. Existing tracking-by-detection methods either ignore this problem, or employ a separate component for managing the training set. We propose a novel generic approach for alleviating the problem of corrupted training samples in tracking-by-detection frameworks. Our approach dynamically manages the training set by estimating the quality of the samples. Contrary to existing approaches, we propose a unified formulation by minimizing a single loss over both the target appearance model and the sample quality weights. The joint formulation enables corrupted samples to be down-weighted while increasing the impact of correct ones. Experiments are performed on three benchmarks: OTB-2015 with 100 videos, VOT-2015 with 60 videos, and Temple-Color with 128 videos. On the OTB-2015, our unified formulation significantly improves the baseline, with a gain of 3.8% in mean overlap precision. Finally, our method achieves state-of-the-art results on all three datasets. Code and supplementary material are available at http://www.cvl.isy.liu.se/research/objrec/visualtracking/decontrack/index.html .

==> relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}
Few discriminative methods employ some form of sample weighting scheme beyond successively downweighting older samples as new ones are gathered. By far the most common method is to simply rely on the tracker being sufficently robust to not gather any signficant number of missaligned/wrong samples. This is a problem for long term occlusions or out-of-view situations. Most commonly used methods will instead reject a sample based on the current tracker confidence, this risks rejecting potentially useful samples, for example the start of a deformation or accepting a potentially wrong sample like a partial occlusion.

The peak to sidelobe ratio used in MOSSE \cite{MOSSE2010} rejects a new sample when the peak to sidelobe ratio, computed as the ratio between the filter output and the remaining samples. This effectively reduces the problem to one of setting the tresholds correctly for rejecting a new sample.

The MEEM tracker stores earlier states of the tracker model and computes the output scores for each stored model in the current frame, if model drift is detected the current tracker is reset to the best of the stored states. Model drift detection and selection of the best model is done using an entropy minimization criterion. In this framework only the currently best fitting model is updated.

Possnegger \cite{Posnegger2015} suggested to train a second classifier using color histograms to filter reduce the influence of regions of similar appreance to the target. However this method is specifically designed to counter problems encountered by color based feature representations, while we primarily use a gradient based feature representation.

%Another approach is to create a second classifier with significantly more background and combine the scores as proposed by \cite{ChaoMa15}.
Another approach proposed by \cite{CahoMa15} et al is to use a pair of classifier, one larger that includes significant background, and a second smaller one with only the target itself, for the smaller target the hann windowing commonly used in correlation trackers to reduce bounduary effects is not used. The smaller model is only updated if the larger model has a sufficently high confidence. In order to counter occlusions a separate random fern classifier is run on the entire image if the tracker confidence gets to low. This classifier is trained online. 

Generative models more commonly employ some form of sample weighting, but unlike discriminative models they usually include a large number of negative samples in their representation. Generative strategies are therfore not very suitable for discriminiative models.

